Reynolds number effect on drag reduction in pipe flows by a transverse wall oscillation

Direct numerical simulations of turbulent pipe flow with transverse wall oscillation (WWO) and with no transverse wall oscillation (NWO) are carried out at friction Reynolds numbers Re{\tau} = 170, 360, and 720. The period and amplitude of the oscillation are selected to achieve high drag reduction in this Reynolds number range, and the effect of increasing Reynolds number on the amount of drag reduction achievable is analyzed. Of a particular interest in this study is the identification of the scales of motion most affected by drag reduction at different Reynolds numbers. To answer this question, both one-dimensional and two-dimensional spectra of different statistical quantities are analyzed with and without transverse wall oscillation. The effect of wall oscillation is found to suppress the intermediate- and large-scale motions in the buffer layer of the flow, while large-scale and very-large-scale motions in the log layer and the wake region are enhanced. While suppression of the near-wall turbulence promotes drag reduction, enhancement of the large-scale motions in the log and the wake region is found to oppose drag reduction. Since higher Reynolds number flows support development of a growing range of large-scale structures, it is suggested that their prevalence in the energy spectra combined with their negative effect on drag reduction account for a reduced effectiveness of wall oscillation as a drag reduction mechanism with increasing Reynolds numbers.

==> backup.tex <==
\iffalse
\begin{equation}
    u_{wall}^+(r=R,\theta,x,t) = U_{wall}^+ \sin{\frac{2\pi}{T_{osc}^+}t^+}.
    \label{eqn:wallbc}
\end{equation}

Figure \ref{fig:pipediag3d} illustrate the domain and boundary conditions of the simulation.  Wall oscillations are prescribed as a velocity boundary condition in the oscillated case.  The velocity is identical everywhere on the pipe wall and varies in time as shown in equation (\ref{eqn:wallbc}).  The velocity of the wall is constant in plus units $U_{wall}^+$ and period $T_{osc}^+$.
\fi

%Experiments have observed that for turbulent flows for which the oscillation period is prescribed that the diffusion of spanwise momentum penetrates only into the beginning or below the buffer layer, the mean azimuthal velocity behaves as a Stokes' layer laminar solution \cite{song2020viscous,coxe2022stokes}.
 \iffalse 
\begin{equation}
    w^+(y^+,t^+) = W_{wall}^+ \Im \left\{ \exp\left(i \frac{2\pi}{T_{osc}^+} t^+ \right) \frac{J_1\left((-1)^{3/4} \sqrt{\pi/T_{osc}^+} (R^+-y^+) \right)}{J_1\left(J_1\left((-1)^{3/4} \sqrt{\pi/T_{osc}^+} R^+ \right)  \right)}\right\}
    \label{eqn:stokesolncyl}
\end{equation}

\begin{equation}
    A^+(y^+,t^+) = \frac{W_{wall}^+ T_{osc}^+}{2\pi} \Re \left\{-i \exp\left(i \frac{2\pi}{T_{osc}^+} t^+ \right) \frac{J_1\left((-1)^{3/4} \sqrt{\pi/T_{osc}^+} (R^+-y^+) \right)}{J_1\left(J_1\left((-1)^{3/4} \sqrt{\pi/T_{osc}^+} R^+ \right)  \right)}\right\}
    \label{eqn:stokeslaydispcyl}
\end{equation}

\begin{figure}
    \centering
    \begin{subfigure}{.35\linewidth}
        \includegraphics[width=0.95\linewidth,center]{wall_phi_32.eps}
        \caption{$\phi = \frac{0\pi}{2} = 2\pi$}
        \label{fig:phase0-32}
    \end{subfigure}%
    \begin{subfigure}{.35\linewidth}
        \includegraphics[width=0.95\linewidth,center]{wall_phi_8.eps}
        \caption{$\phi = \frac{\pi}{2}$}
        \label{fig:phase8}
    \end{subfigure}
    ~
    \begin{subfigure}{.35\linewidth}
        \includegraphics[width=0.95\linewidth,center]{wall_phi_16.eps}
        \caption{$\phi = \pi$}
        \label{fig:phase16}
    \end{subfigure}%
    \begin{subfigure}{.35\linewidth}
        \includegraphics[width=0.95\linewidth,center]{wall_phi_24.eps}
        \caption{$\phi = \frac{3\pi}{2}$}
        \label{fig:phase24}
    \end{subfigure}\quad
    \caption{Illustration of four phases of the pipe oscillation: a.)  $\phi = \frac{0\pi}{2} = 2\pi$, b.) $\phi = \frac{\pi}{2}$ c.) $\phi = \pi$ d.$\phi = \frac{3\pi}{2}$) .  The solid blue arrow indicates the wall velocity and the dashed blue box indicates the wall position.  Naturally, the wall phase lags $90^\circ$ behind.  The amplitude of wall displacement in viscous units is $\nicefrac{1000}{2 \pi} \approx 160$}
    \label{fig:wallphase}
\end{figure}


Equation \ref{eqn:stokesolncyl} (\cite{song2020viscous,coxe2022stokes}) gives the azimuthal velocity profile in viscous units as a function of wall normal location and time for a pipe.  In the limit as Reynolds number goes to infinity the stokes layer becomes thinner with respect to the overall radius.  Additionally, the displacement of the wall can be readily integrated in time to be shown to be equation \eqref{eqn:stokeslaydispcyl}.  In this equation, the parameter values all come from the original boundary condition equation \ref{eqn:wallbc}.

\begin{equation}
	\delta^+ = 4.5 \left( \frac{T_{osc}^+}{\pi} \right)^{1/2}
	\label{eqn:stokesthick}
\end{equation}

Given by \ref{eqn:stokesthick} is the distance that this stokes layer penetrates into the mean streawmise flow in wall units.  The definition of $\delta^+$ comes from equation flat plate solution when the decaying exponential $e^{-\sqrt{\nicefrac{\pi}{T_{osc}^+}}y^+}$ is equal to $0.01$.


Due to this periodic variation in the azimuthal velocity, turbulent fluctuations are calculated with respect to a particular phase.  Wall phase angle refers to the integer fraction of the oscillation period as either $\phi = \frac{n T_{osc}}{N}$ or $\phi = \frac{n 2 \pi}{N}$.  Figure \ref{fig:wallphase} explains, graphically, what is meant by wall phase angle.  The solid blue arrow in figure \ref{fig:phase0-32} illustrates a phase of $\phi = 0, 2\pi$.  Phase is determined by the wall velocity function only and not the wall displacement.  At this location the wall has displaced itself furthest in the clockwise direction.  At maximum wall velocity, the wall experiences zero displacement.  Mean statistics in drag reduction are separated by phase angle of the wall velocity and not the wall displacement.  Figures \ref{fig:phase16} and \ref{fig:phase24} illustrate the second half of the wall oscillation period for completeness and thus show maximum anti-clockwise displacement and a return to zero displacement. 
\fi


\iffalse
\subsection{Fukagata-Iwamoto-Kasagi Identity}\label{sec:fik}
The Fukagata-Iwamoto-Kasagi (FIK) identity, relates the contribution of turbulence to the overall reduction in wall shear stress, $U_{bulk}$ \cite{fukagata2002contribution}. Extension of this to bulk contribution - find and cite it. Write FIK through single integral.

\begin{equation}
    \frac{U_{bulk}}{\utau} = \frac{\ret}{4} - \frac{\ret}{\utau^2} \int_0^1   \ava{\upp \vpp} \rstar^2 d\rstar
\end{equation}

Where $\ubulk = 2 \int_0^1 \ava{u_x} \rstar d\rstar$, $\rstar=\frac{r}{R}$, and $\ret = \frac{u_\tau R}{\nu}$. 
\iffalse
The turbulent fluctuations $\upp$ and $\vpp$ are the triply decomposed fluctuations by method Hussain and Reynolds\cite{hussain1970mechanics}.
\begin{equation}
    u_i = \at{u_i} + u_i^\phi + u_i^\dpr
    \label{eqn:tripledecomp}
\end{equation}
here $u_i^\phi$ is the periodic component of fluctuation which varies with wall oscillation and is decomposed by averaging over snapshots with oriented with phase angles described by figures \ref{fig:phase0-32}.
\fi
Define laminar and turbulent contribution. 
Define $U_{bulk}$ turbulent cumulative. 
%where the sum over all wave numbers of the co-spectra of streamwise and radial velocities results in the co-variance of streamwise-radial velocity or the Reynolds shear stress.  
Turbulent contribution to $U_{bulk}$ is defined as (cite Fukagata)
\begin{equation}
    \frac{U_{bulk}^{t,cum}}{u_\tau} = -\frac{\ret}{\utau^2} \int_{1-y}^1 \ava{\upp \vpp} r^\star dr^\star
\end{equation}
and then explain what it means.

One can consider the definition of the Reynolds stress by means of Fourier modes (see also, e.g., cite Chan):

\begin{equation}
    \upp \vpp = \sum_{m,n} \hat{\upp \vpp}(k_m,k_n,r,t) \exp{\left(-i(k_m x + k_n \theta)\right)} 
\end{equation}
Don't go discrete.

where $k_m = 2\pi \frac{m}{L}$ and $k_n = 2\pi n$.  The $(m,n)$ fourier mode of the Reynolds stress spectra is given by the convolution:
\begin{equation}
    \reallywidehat{\upp \vpp}(k_m,k_n,r,t) = \sum_{k_p} \sum_{k_q} \sum_{k_r} \sum_{k_j} \upph(k_p,k_q,r,t) \vpph(k_r,k_j,r,t)\delta_{p+r,m} \delta_{q+j,n}
\end{equation}

The averaging operator in the streamwise and azimuthal directions is the equivalent of the inner product with the zeroth fourier mode which by orthogonality results in 

\begin{equation}
    \avxt{\upp \vpp} = \reallywidehat{\upp \vpp}(k_m=0,k_n=0,r,t) = \sum_{k_p} \sum_{k_q} \upph(k_p,k_q,r,t) \vpph(-k_p,-k_q,r,t)
\end{equation}
By definition of the velocity field being a real-valued function, the spectra is hermitian resulting the streamwise average of the Reynolds shear-stress being equal to the sum over the co-spectra of $\upp$ and $\vpp$.

\begin{equation}
    \frac{\ubulk}{\utau} = 
    \frac{\ret}{4} - 
    \frac{\ret}{\utau^2} \int_0^1 
    \int_0^\rstar 
    \frac{1}{\gamma} 
    \frac{\partial \gamma \sum_{k_p} \sum_{k_q} \at{ S_{\uc,\vc} (k_p,k_q,\gamma,t} }{\partial \gamma} \gamma d\gamma \rstar d\rstar
\end{equation}

The double integral over the pipe radius of the net force due to the Reynolds shear stress can be shown, through integration by parts to be represented by a single integral 

\begin{equation}
    \frac{U_{bulk}}{u_\tau} = \frac{Re_\tau}{4} - \frac{\ret}{\utau^2}\sum_{k_x} \sum_{k_\theta} \int_0^1 \at{S_{\uc \vc}} {r^\star}^2 d r^\star
\end{equation} 

Add a formula for $U_{bulk}$ cumulative through wave numbers.

%This relationship follows from Parseval's theorem\citep{rayleigh1889liii}.  Note, that this relationship between FIK identity and the co-spectra of $\upp$ and $\vpp$ was introduced by \cite{chan2022large} who arrived at this representation through application of a full convolution of the wave number matrix and showing that this relation ship can be arrived at by showing that contribution from cross terms decreases with $\frac{1}{\mid \Delta k \mid^2}$ for the full convolution.
\fi


To provide a better understanding of what is occuring at this wavelength we observe the streamwise-azimuthal spectrum of $u_x^{\prime \prime}$ located half-way between these two wall normal coordinates of interest shown in figure \ref{fig:DeltaUUyp15AzmStw}.

\begin{figure}
    \begin{subfigure}{0.325\linewidth}
        \includegraphics[width=0.99\linewidth]{figures/spectraUU/stw_azm_Duu_170_yp015.pdf}
        \caption{$Re_\tau = 170$}
        \label{fig:DuuAzmStwyp15Re170}
    \end{subfigure}
    \begin{subfigure}{0.325\linewidth}
        \includegraphics[width=0.99\linewidth]{figures/spectraUU/stw_azm_Duu_360_yp015.pdf}
        \caption{$Re_\tau = 360$}
        \label{fig:DuuAzmStwyp15Re360}
    \end{subfigure}
    \begin{subfigure}{0.325\linewidth}
        \includegraphics[width=0.99\linewidth]{figures/spectraUU/stw_azm_Duu_720_yp015.pdf}
        \caption{$Re_\tau = 720$}
        \label{fig:DuuAzmStwyp15Re720}
    \end{subfigure}
    \caption{Change in the streamwise energy spectra located at $y^+=15$.  This location is chosen as a midway point to isolate the changes imparted in the azimuthal spectrum of streamwise velocity as a result of WWO.  A large scale roll mode at this very large streamwise and azimuthal wavelengths is observed and that increasing Reynolds number enhances the energy in these modes.}
    \label{fig:DeltaUUyp15AzmStw}
\end{figure}
These contours of the change in the streamwise-azimuthal energy spectra illustrate the impact of Reynolds number on wavelengths of motion.  Clearly as the Reynolds number increases, large scales become more energetic.  However there remains band of suppression of streaky long streaky structures in the buffer-layer as observerd by the blue band around azimuthal arc lengths of $r^+ \lambda_\theta \approx 100$.  This effect is diminishes as Reynolds number increases.  Black lines indicate the angle associate with very large scale roll modes\cite{wu2012direct} while the orange dotted lines are the range of angles associated with the meandering of large scale structures.  Wall oscillations do not appear to impact the meandering of large scale streaks but do appear to allow very large scale roll modes to penetrate further to the wall.  Likely due to the suppression of near-wall turbulence which would otherwise break them up.

\iffalse
\begin{table}[]
    \centering
    \begin{tabular}{  c c c c}
         $\ret$ & NWO/WWO   & $ \Delta$  & NWO/WWO   & $ \Delta$  & NWO/WWO & $ \Delta$   \\ 
          & \multicolumn{2}{c}{total}   &  \multicolumn{2}{c}{lpf} &  \multicolumn{2}{c}{hpf}  \\ \hline
         170 & 13.7/15.7 & 2 & 14.3/19.0 & 4.7 & 13.0/14.6 & 1.6 \\
         360 & 13.9/15.7 & 1.8 & 14.8/19.7 & 4.9 & 13.1/14.4 & 1.3 \\
         720 & 14.5/16.1 & 1.6 & 15.5/20.8 & cite5.3 & 13.5/14.6 & 1.1
    \end{tabular}
    \caption{Wall normal location ($y^+$) at which the net turbulent force changes from accelerating the mean flow to decelerating the mean flow, along with the difference between the WWO and NWO locations ($\Delta$).}
    \label{tab:fturbzero}
\end{table}
\fi
